Simplicial volume of open books in dimension 4

In this short note we adapt a proof by Bucher and Neofytidis to prove that the simplicial volume of 4-manifolds admitting an open book decomposition vanishes. In particular this shows that Quinns signature invariant, which detects the existence of an open book decomposition in dimensions above 4, is insufficient to characterize open books in dimension 4, even if one allows arbitrary stabilizations via connected sums.

==> Corollary/AcyclicImpliesUBC.tex <==
\begin{corollary}
\label{cor:AcyclicUBC}
  Let $\TopologicalSpace$ denote a connected topological space such that
  $
    \BoundedCohomologyOfSpaceObject
      {q+1}
      {\HomotopyGroupOfObject{1}{\TopologicalSpace}{\ast}}
      {\Reals}
  $
  vanishes, then $\TopologicalSpace$ satisfies the $q$-UBC.
\end{corollary}

==> Definition/UBC.tex <==
\begin{definition}[Definition~SOMETHING in \cite{MatsumotoMorita}]
  Let $\TopologicalSpace$ denote a topological space. We say
  $\TopologicalSpace$ satisfies the $q$-uniform boundary condition ($q$-UBC) if
  there exists a constant $K$ such that for every closed singular $q$-chain
  with real coefficients $\sigma$ on $\TopologicalSpace$ that is a boundary,
  there exists a
  $q+1$-chain $\rho$ on $\TopologicalSpace$ such that $\partial \rho = \sigma$
  and $\Norm{\rho}\leq K \Norm{\sigma}$.
\end{definition}

==> Lemma/BoundingCycle.tex <==
\begin{lemma}
\label{lem:BoundingCycle}
  Let $\NullBordism$ denote an oriented $n+1$-dimensional compact manifold with
  boundary $\Manifold$ and let $\FundamentalCycle{\Manifold}$ denote a
  fundamental cycle of $\Manifold$. Then any $n+1$-chain
  $\FundamentalCycle{\NullBordism,\Manifold}$ on $\NullBordism$ that bounds
  $\FundamentalCycle{\Manifold}$ represents the fundamental class of
  $(\NullBordism,\Manifold)$.
\end{lemma}
\begin{proof}
  The boundary morphism of the long exact sequence of the pair
  $(\NullBordism,\Manifold)$ maps an $(n+1)$-chain on the pair
  $(\NullBordism,\Manifold)$ to its boundary in $\Manifold$. Hence the homology
  class represented by $\FundamentalCycle{\NullBordism,\Manifold}$ maps to the
  class represented by $\FundamentalCycle{\Manifold}$ i.e. the fundamental
  class of $\Manifold$. Therefore it represents the fundamental class of
  $(\NullBordism,\Manifold)$.
\end{proof}

==> Lemma/FiberTransfer.tex <==
\begin{lemma}
\label{lem:FiberTransfer}
  Let $\pi\colon \ManifoldTotal \to \ManifoldBase$ denote a fiber bundle with
  fiber $\ManifoldFiber$ being a
  manifold with a potentially empty
  boundary such that $\ManifoldFiber$ and $\Boundary{\ManifoldFiber}$ are
  connected (or empty) and both have amenable fundamental group, then there
  exists chain maps
  \[
    \FiberTransferHomology{\pi}_{d}
    \colon
    C_d(\ManifoldBase)
    \to
    C_{d+f}(\ManifoldTotal, \Boundary{\ManifoldTotal})
  \]
  where $f$ denotes the dimension of the fiber and $\Boundary{\ManifoldTotal}$
  denotes the restriction of the bundle to the fiberwise boundary, of
  degreewise arbitrarily small norm realizing the fiber transfer
  \[
    \HomologyOfSpaceObject{d}{\ManifoldBase}{\Reals}
    \to
    \HomologyOfSpaceObject{d+f}{\ManifoldTotal,\Boundary{\ManifoldTotal}}{\Reals}
  \]
  on the chain level.
\end{lemma}
\begin{proof}
  Fix a fundamental cycle
  $
    \FundamentalCycle{\ManifoldFiber, \Boundary{\ManifoldFiber}}
  $
  of arbitrarily small norm and for every point in $\ManifoldBase$ a
  trivialization of the fiber over that point (These do not have to satisfy any
  compatibility conditions, they are truly arbitrary).
  Now define
  $\FiberTransferHomology{\pi}_0$ to be the
  image of $\FundamentalCycle{\ManifoldFiber, \Boundary{\ManifoldFiber}}$ under
  the aforementioned arbitrary trivializations.

  We now proceed inductively. Suppose we are able to construct maps
  $\FiberTransferHomology{\pi}_{n-1}$ of arbitrary small norm representing the
  fiber transfer and that
  $\apply{\pi_{d}}{\Simplex{d}}$ is supported
  on $\at{\ManifoldTotal}{\Simplex{d}}$ for any singular simplex $\Simplex{d}$.
  Let $\Simplex{n}$ denote a singular $n$-simplex in $\ManifoldBase$. Then
  $
    \Boundary
      {
        \apply
          {\FiberTransferHomology{\pi}_{n-1}}
          {\Boundary{\Simplex{n}}}
      }
  $
  is a fundamental cycle of
  $\at{\Boundary{\ManifoldTotal}}{\Boundary{\Simplex{n-1}}}$.
  Let $K_1$ denote the UBC constant in degree $n+f-2$ of
  $
    \StandardSimplex{n} \times \Boundary{\ManifoldFiber}
  $%
  , which exists because the fundamental group of $\Boundary{\ManifoldFiber}$
  is amenable. Let $\rho_{\Simplex{n}}$ denote a filling of
  $
    \Boundary
    {
      \apply
      {\FiberTransferHomology{\pi}_{n-1}}
      {\Boundary{\Simplex{n}}}
    }
  $
  in $\at{\ManifoldTotal}{\Simplex{n-1}}\times \Boundary{\ManifoldFiber}$ such
  that
  \[
    \Norm{\rho_{\Simplex{n}}}
    \leq
    K_1
    \Norm{
      \Boundary
        {
          \apply
            {\FiberTransferHomology{\pi}_{n-1}}
            {\Boundary{\Simplex{n}}}
        }
    }
  \]
  Now
  $
    \apply
      {\FiberTransferHomology{\pi}_{n-1}}
      {\Boundary{\Simplex{n}}}
    +
    \rho_{\Simplex{n}}
  $
  represents a fundamental cycle of $\Boundary{\Simplex{n}\times
  \ManifoldFiber}$ by Lemma~\ref{lem:BoundingCycle}.
  Let $K_2$ denote the UBC constant of
    $
      \Simplex{n}
      \times
      \ManifoldFiber
    $
    in degree $n+f-1$, then there exists a filling $P_{\Simplex{n}}$ of
    $
      \apply
        {\FiberTransferHomology{\pi}_{n-1}}
        {\Boundary{\Simplex{n}}}
      +
      \rho_{\Simplex{n}}
    $
    such that
    \[
      \Norm{P_{\Simplex{n}}}
      \leq
      K_2
      \Norm
        {
          \apply
            {\FiberTransferHomology{\pi}_{n-1}}
            {\Boundary{\Simplex{n}}}
          +
          \rho_{\Simplex{n}}
        }
      \leq
      K_2
      \left(
        (n+1)\Norm{\FiberTransferHomology{\pi}_{n-1}}
        +
        K_1
        (n+1)n\Norm{\FiberTransferHomology{\pi}_{n-1}}
      \right)
    \]
    Since $\Norm{\FiberTransferHomology{\pi}_{n-1}}$ can be chosen to be
    arbitrarily small, we conclude by Lemma~\ref{lem:BoundingCycle} that this
    yields the desired extensions of arbitrarily small norm.
\end{proof}

==> Lemma/FreeGroupUBC.tex <==
\begin{lemma}
\label{lem:FreeGroupUBC}
  Let $n\geq4$.
  Suppose $\BoundedCohomologyOfSpaceObject{n}{\FreeGroup{k}}{\Reals}$ is
  zero, and let $\Manifold$ denote a manifold that is obtained from
  $
    \#_k
    \Sphere{1}\times \Sphere{n-1}
  $
  by a finite number of disjoint $1$-surgeries i.e. there exists embeddings
  $
    \HandleEmbedding^i
    \colon
    \Sphere{1} \times \Ball{n-1}
    \to
    \#_k
    \Sphere{1}\times \Sphere{n-1}
  $
  such that
  \[
    \#_k
    \Sphere{1} \times \Sphere{n-1}
    \setminus
    \left(
      \bigsqcup_i
      \apply
        {\HandleEmbedding^{i}}
        {\Sphere{1}\times\Inner{\Ball{n-1}}}
    \right)
    \cup
    \bigsqcup_i
    \Ball{2} \times \Sphere{n-2}
    =
    \Manifold
  \]
  Then the simplicial volume of $\Manifold$ vanishes.
\end{lemma}
\begin{proof}
  By assumption $\Manifold$ splits as
  \[
    \Manifold
    =
    \#_k
    \Sphere{1} \times \Sphere{n-1}
    \setminus
    \left(
      \bigsqcup_i
      \apply
        {\HandleEmbedding^{i}}
        {\Sphere{1}\times\Inner{\Ball{n-1}}}
    \right)
    \cup_{\bigsqcup \apply{\HandleEmbedding^i}{\Sphere{1} \times \Sphere{n-2}}}
    \Ball{2}\times\Sphere{n-2}
  \]
  Since $\Ball{2}\times \Sphere{n-2}$ is simply-connected, the disjoint
  union has vanishing bounded cohomology in all positive degrees.
  Since the dimension is at least $4$, we conclude by transversality that the
  fundamental group of
  $
    \#_k
    \Sphere{1} \times \Sphere{n-1}
    \setminus
    \left(
      \bigsqcup_i
      \apply
      {\HandleEmbedding^{i}}
      {\Sphere{1}\times\Inner{\Ball{n-1}}}
    \right)
  $
  is still a free group on $k$ generators.

  Hence by Corollary~\ref{cor:AcyclicUBC}, both
  $
    \#_k
    \Sphere{1} \times \Sphere{n-1}
    \setminus
    \left(
      \bigsqcup_i
      \apply
        {\HandleEmbedding^{i}}
        {\Sphere{1}\times\Inner{\Ball{n-1}}}
    \right)
  $
  and
  $
    \bigsqcup_i
    \Ball{2}\times \Sphere{n-2}
  $
  satisfy $(n-1)$-UBC. Furthermore the simplicial volume of $\Sphere{1}\times
  \Sphere{n-2}$ vanishes, hence by Lemma~\ref{lem:UBCGluing}, the simplicial
  volume of $\Manifold$ vanishes.
\end{proof}

==> Lemma/SurgerySimplicialVolume.tex <==
\begin{lemma}
\label{lem:Surgery}
  Let $\Manifold$ and $\ManifoldAlternative$ denote manifolds of dimension at
  least $4$. Suppose further that
  $\ManifoldAlternative$ is obtained from $\Manifold$ by $k$-surgery at
  $\HandleEmbedding\colon \Sphere{k} \times \Ball{n-k} \to \Manifold$ for some
  $k\in \{-1, 0, \ldots, n\}$
  i.e.
  $
    \ManifoldAlternative
    =
    \Manifold
    \setminus
    \apply{\HandleEmbedding}{\Sphere{k}\times \Inner{\Ball{n-k}}}
    \cup_{\apply{\HandleEmbedding}{\Sphere{k}\times \Sphere{n-k-1}}}
    \Ball{k+1}\times \Sphere{n-k-1}
  $%
  , then:
  \begin{itemize}
  \item
    If $k \not \in \{1, n-2\}$, then $\SimplicialVolume{\Manifold} =
    \SimplicialVolume{\ManifoldAlternative}$
  \item
    If $k=1$, then
    $
      \SimplicialVolume{\ManifoldAlternative}
      \leq
      \SimplicialVolume{\Manifold}
    $
  \item
    If $k=n-2$, then
    $
      \SimplicialVolume{\Manifold}
      \leq
      \SimplicialVolume{\ManifoldAlternative}
    $
  \end{itemize}
\end{lemma}
\begin{proof}
  First of all, if $\Manifold$ is obtained from $\ManifoldAlternative$ by a
  $k$-surgery, then $\ManifoldAlternative$ is obtained from $\Manifold$ by a
  $n-k-1$-surgery. Hence we only have to consider either the case $k$ or
  $n-k-1$ and obtain the other via this symmetry. Note that since $n\geq 4$
  this does not cause any issues.

  Now for $k = -1$ we have $\ManifoldAlternative = \Manifold \cup \Sphere{n}$.
  Hence $\SimplicialVolume{\ManifoldAlternative} =
  \SimplicialVolume{\Manifold}$.

  For $k=0$, there are two cases two consider:
  The embedding $\Sphere{0} \times \Ball{n} \to \Manifold$, might hit the same
  or two different connected components of $\Manifold$. In the first case we
  have $\ManifoldAlternative \cong \Manifold \# \Sphere{1} \times \Sphere{n-2}$
  and in the second case we have
  $
    \ManifoldAlternative
    =
    \Manifold_1
    \#
    \Manifold_2
  $
  for $\Manifold_i$ a corresponding splitting of the connected components of
  $\Manifold$. In both cases the simplicial volume does not change by Gromovs
  Additivity Theorem.

  Now let us consider  $k\in \{2,\ldots, n-3\}$ and let
  $
    \HandleEmbedding
    \colon
    \Sphere{k}
    \times
    \Ball{n-k}
    \to
    \Manifold
  $
  denote an embedding. Let
  \[
    \Bordism =
    \Manifold \times [0,1]
    \cup_{\apply{\HandleEmbedding}{\Sphere{k}\times\Ball{n-k}}}
    \Ball{k}\times\Ball{n-k+1}
  \]
  denote the trace of the surgery at $\HandleEmbedding$.
  Since $\Sphere{k}\times \Ball{n-k}$ is simply-connected, we conclude by
  Seifert-Van-Kampen that
  $
    \HomotopyGroupOfObject{1}{\Bordism}{\ast}
    =
    \HomotopyGroupOfObject{1}{\Manifold}{\ast}
  $%
  . By flipping the role of $\Manifold$ and $\ManifoldAlternative$ and using
  that $n\geq 4$ and $k\leq n-3$, we also obtain
  $
    \HomotopyGroupOfObject{1}{\Bordism}{\ast}
    =
    \HomotopyGroupOfObject{1}{\ManifoldAlternative}{\ast}
  $%
  . Hence the following diagram commutes
  \[
    \begin{tikzcd}
      \Manifold
        \ar[d]
        \ar[dr]
      \\
      \Bordism
        \ar[r]
      &
      \ClassifyingSpace{\HomotopyGroupOfObject{1}{\Manifold}{\ast}}
      \\
      \ManifoldAlternative
        \ar[u]
        \ar[ur]
    \end{tikzcd}
  \]
  where both diagonal maps represent the classifying maps of their respective
  universal coverings. Hence $\Manifold$ and $\ManifoldFiber$ map their
  fundamental classes to the same homology class in
  $
    \ClassifyingSpace{\HomotopyGroupOfObject{1}{\Manifold}{\ast}}
    =
    \ClassifyingSpace{\HomotopyGroupOfObject{1}{\ManifoldAlternative}{\ast}}
  $%
  . Therefore by Gromovs Mapping Theorem their simplicial volumes agree.

  Finally let us consider $k=n-2$: Let
  $
    \HandleEmbedding
    \colon
    \Sphere{n-2} \times \Ball{2}
    \to
    \Manifold
  $
  denote an embedding. Let us again consider the trace of the surgery at
  $\HandleEmbedding$:
  \[
    \Bordism =
    \Manifold \times [0,1]
    \cup_{\apply{\HandleEmbedding}{\Sphere{n-2}\times\Ball{2}}}
    \Ball{n - 2 + 1}\times\Ball{2}
  \]
  Again we conclude via Seifert-Van-Kampen that
  $
    \HomotopyGroupOfObject{1}{\Bordism}{\ast}
    =
    \HomotopyGroupOfObject{1}{\Manifold}{\ast}
  $
  hence the following diagram commutes as well
  \[
    \begin{tikzcd}
      \Manifold
        \ar[d]
        \ar[dr,"g"]
      \\
      \Bordism
        \ar[r]
      &
      \ClassifyingSpace{\HomotopyGroupOfObject{1}{\Manifold}{\ast}}
      \\
      \ManifoldAlternative
        \ar[u]
        \ar[ur, "f"]
    \end{tikzcd}
  \]
  where the upper diagonal map $g$ represents the universal covering of
  $\Manifold$
  and the lower diagonal map $f$ is given by the concatenation of the inclusion
  $\ManifoldAlternative \hookrightarrow \Bordism$ and the map representing
  the universal covering of $\Bordism$.
  Hence we have
  $
    \apply{g_*}{\FundamentalClass{\Manifold}}
    =
    \apply{f_*}{\FundamentalClass{\ManifoldAlternative}}
  $
  and therefore
  \[
    \SimplicialVolume{\Manifold}
    =
    \Norm{\apply{g_*}{\FundamentalClass{\Manifold}}}
    =
    \apply{f_*}{\FundamentalClass{\ManifoldAlternative}}
    \leq
    \SimplicialVolume{\ManifoldAlternative}
  \]
\end{proof}

==> Lemma/UBCimpliesSimplicialVolume.tex <==
\begin{lemma}
\label{lem:UBCGluing}
  Suppose a closed connected $n$-dimensional manifold $\Manifold$ splits as
  $
    \Manifold
    =
    \Manifold_1
    \cup_{\Submanifold}
    \Manifold_2
  $
  with $\Manifold_1$ and $\Manifold_2$ being two codimension $0$ submanifolds
  with boundary, that intersect in their common boundary
  $\Submanifold$. Suppose further that
  $\SimplicialVolume{\Manifold_2,\Submanifold}$
  vanishes and $\Manifold_1$ satisfies $(n-1)$-UBC, then the
  simplicial volume of $\Manifold$ vanishes.
\end{lemma}
\begin{proof}
  Let $(\FundamentalCycle{\Manifold_2}^{k})_{k\in\NaturalNumbers}$ denote a
  sequence of fundamental cycles of $\Manifold_2,\Boundary{\Manifold_2}$ such
  that
  $\Norm{\FundamentalCycle{\Manifold_2}^{k}}$ tends to zero as $k$ tends to
  infinity.
  Let $K_1$ denote the UBC-constant in dimension $n-1$ of $\Manifold_1$. Now by
  $(n-1)$-UBC there exist an $n$-chain
  $\FundamentalCycle{\Manifold_1}^{k}$ on
  $\Manifold_1$ that bounds $\Boundary{\FundamentalCycle{\Manifold_2}^k}$
  and such that
  \[
    \Norm{\FundamentalCycle{\Manifold_1}^{k}}
    \leq
    K_1
    \Norm{\Boundary{\FundamentalCycle{\Manifold_2}^{k}}}
    \leq
    (n+1)K_1\Norm{\FundamentalCycle{\Manifold_2}^{k}}
  \]
  By Lemma~\ref{lem:BoundingCycle},
  $\FundamentalCycle{\Manifold_1}^{k}$ represents the fundamental
  class of $\Manifold_1,\Boundary{\Manifold_1}$.
  The difference of $\FundamentalCycle{\Manifold_1}^{k}$ and
  $\FundamentalCycle{\Manifold_2}^{k}$ is closed and therefore represents the
  fundamental class of $\Manifold$. Since the norm of
  $\FundamentalCycle{\Manifold_1}^{k}$ tends to zero, the norm of these
  differences tends to zero as well.
\end{proof}

==> Proof/Existence.tex <==
\begin{proof}[Proof of Proposition~\ref{prp:Existence}]
  Let $\Manifold$ denote a connected $n$-dimensional manifold with non-zero
  simplicial volume. By potentially replacing $\Manifold$ by
  $
    \Manifold
    \#
    -\Manifold
  $
  we can assume that $\Manifold$ is nullbordant. Let $\NullBordism$ denote a
  connected bordism between $\Manifold$ and $\Sphere{n}$. By standard
  arguments, i.e. the existence of a self-indexing Morse function,
  $\NullBordism$ admits a handlebody decomposition relative to $\Sphere{n}$ of
  the following form: There exists
  $
    i_0
    =
    1
    \leq
    i_1
    \leq
    \ldots
    \leq
    i_{n-1}
    \leq
    i_n = k
  $
  such that
  \[
    \NullBordism
    =
    \Sphere{n}\times [0,1]
    +
    \HandleEmbedding^{1}
    +
    \ldots
    +
    \HandleEmbedding^{k}
  \]
   where $\HandleEmbedding^{l}$ denotes an embedding
  \[
    \Sphere{p}
    \times
    \Ball{n-p}
    \to
    \partial \Bordism
    +
    \HandleEmbedding^{1}
    +
    \ldots
    +
    \HandleEmbedding^{l-1}
  \]
  if $l \in [i_p, i_{p-1})$. In particular this shows that
  $\Manifold$ is obtained from $\Sphere{n}$ by a sequence of surgeries of
  increasing index.
  Furthermore since the bordism was assumed to be connected, we can assume that
  there are no $-1$-surgeries and $n$ surgeries.

  Let us denote by $\Manifold_{p}$ the result of performing the surgery for all
  indices less or equal than $p$.
  We readily obtain
  $
    \Manifold_{0}
    =
    \#_{i_1}
    \Sphere{1}\times\Sphere{n-1}
  $%
  and
  $
    \Manifold = \Manifold_{n-1}
  $
  . On the other side, by Lemma~\ref{lem:Surgery} we obtain
  \[
    0
    \leq
    \SimplicialVolume{\Manifold}
    =
    \SimplicialVolume{\Manifold_{n-2}}
    \leq
    \SimplicialVolume{\Manifold_{n-3}}
    =
    \ldots
    =
    \SimplicialVolume{\Manifold_{1}}
  \]
  Now note that performing surgery at isotopic embeddings, yields diffeomorphic
  manifolds. Since the dimension is assumed to be at least $4$, we can hence
  assume via transversality that the embeddings for the $1$-surgeries are all
  disjoint. Hence
  $
    \Manifold_{1}
  $
  has the desired property.
\end{proof}

==> Proposition/ComplementGeometricDimension.tex <==
\begin{proposition}
\label{prp:Complement}
  Let $\Manifold$ denote a closed manifold of dimension $\Dimension \geq 3$.
  Suppose $\Submanifold\subset \Manifold$ is a simply-connected codimension $2$
  submanifold,
  such that there exists a classifying space for
  $\HomotopyGroupOfObject{1}{\Manifold\setminus\Submanifold}{\Point}$ of
  dimension at most $n-1$, then $\Manifold$ is inessential.
\end{proposition}

==> Proposition/ExistenceManifold.tex <==
\begin{proposition}
\label{prp:Existence}
  Let $n\geq 4$, then there exists an $n$-dimensional oriented closed connected
  manifold $\Manifold$ with non-vanishing simplicial volume and $\Manifold$
  is obtained from $\#_k \Sphere{1}\times \Sphere{n-1}$ for some $k$ by a
  finite number of disjoint $1$-surgeries.
\end{proposition}


==> Proposition/FreeGroupRankIrrelevant.tex <==
\begin{proposition}
  Let $n$ denote a natural number or infinity and suppose that
  $\BoundedCohomologyOfSpaceObject{k}{\FreeGroup{n}}{\Reals}$ is non-zero ,
  then $\BoundedCohomologyOfSpaceObject{k}{\FreeGroup{n'}}{\Reals}$ is
  non-zero for any other $n' \geq 2$ and the rank of
  $\BoundedCohomologyOfSpaceObject{k}{\FreeGroup{*}}{\Reals}$ is infininite
  dimensional.
\end{proposition}
\begin{proof}
 It follows from Theorem~6.14 in \cite{DGO} that free groups contain all other
 free groups as hyperbolically embedded subgroups, hence by Corollary~2 in
 \cite{FrigerioPozettiSisto} we conclude that if the bounded cohomology of one
 free group is non-zero in degree $k$, then it is non-zero for all non-abelian
 free groups.

 Now in order to show that its rank is infinite consider the following two maps:
 $f$ is given as the inclusion of $\Sphere{1} \vee \Sphere{1} \hookrightarrow
 \bigvee_4 \Sphere{1}$ as the first two circles and $g$ is given as the map $
 \bigvee_4 \Sphere{1} \to \Sphere{1} \vee \Sphere{1}$ that collapses the first
 two circles. Since $g$ has a section it induces an injective map on bounded
 cohomology and because $f$ is a retract it induces a surjective map on bounded
 cohomology. The composition $g\circ f$ is null-homotopic, hence induces the
 zero map on bounded cohomology. From that we obtain that
 \[
    \apply
      {\textrm{rk}}
      {\BoundedCohomologyOfSpaceObject{k}{\FreeGroup{4}}{\Reals}}
    \geq
    2
    \apply
      {\textrm{rk}}
      {\BoundedCohomologyOfSpaceObject{k}{\FreeGroup{2}}{\Reals}}
  \]
  because the image of the map induced by $g$ is orthogonal to a preimage of
  the bounded cohomology of $\FreeGroup{2}$ under $f$.
  Nevertheless by Corollary~2 in \cite{FrigerioPozettiSisto} we have
  \[
    \apply
      {\textrm{rk}}
      {\BoundedCohomologyOfSpaceObject{k}{\FreeGroup{4}}{\Reals}}
    \leq
    \apply
      {\textrm{rk}}
      {\BoundedCohomologyOfSpaceObject{k}{\FreeGroup{2}}{\Reals}}
  \]
  Combining these two inequalities yields the desired result.
\end{proof}

==> Proposition/MappingTori.tex <==
\begin{proposition}
\label{prp:MappingTori}
  Let
  $
    \Diffeomorphism
    \colon
    \left(\Manifold,\Boundary{\Manifold}\right)
    \to
    \left(\Manifold,\Boundary{\Manifold}\right)
  $
  denote an arbitrary diffeomorphism of some compact
  $3$-manifold $\Manifold$ that restricts to the identity on the boundary.
  Suppose further that the fourth bounded cohomology of non-abelian free groups
  vanishes, then the relative simplicial volume of the mapping tori
  $\MappingTorus{\Diffeomorphism}$ vanishes
\end{proposition}

==> Proposition/MatsumotoMorita.tex <==
\begin{proposition}[Proposition~SOMETHING in \cite{MatsumotoMorita}]
\label{prp:MatsumotoMorita}
  A topological space satisfies $\TopologicalSpace$ satisfies the $q$-UBC if
  and only if the comparison map
  \[
    \BoundedCohomologyOfSpaceObject{q+1}{\TopologicalSpace}{\Reals}
    \to
    \CohomologyOfSpaceObject{q+1}{\TopologicalSpace}{\Reals}
  \]
  is injective.
\end{proposition}

==> Proposition/NeighborhoodImmersedCodim2.tex <==
\begin{proposition}
\label{prp:GeneralizedTubNeighborhood}
  Let $\Manifold$ denote an $n$-manifold and
  $
    \ContinuousMap
    \colon
    \Submanifold
    \to
    \Manifold
  $
  an immersion such that there exists an embedded submanifold
  $\Singularity_{mp} \subset \Submanifold$ with the properties:
  \begin{enumerate}[(i)]
  \item
    the restriction of $\ContinuousMap$ to $\Submanifold \setminus
    \Singularity_{mp}$ is injective.
  \item
    the image of $\Singularity_{mp}$ and $\Submanifold \setminus
    \Singularity_{mp}$ are disjoint
  \item
    every point in $\apply{\ContinuousMap}{\Singularity_{mp}}$ has exactly two
    preimages and the corresponding tangent spaces intersect transversally.
  \end{enumerate}
  then there exists a closed neighborhood $\TubularNeighborhood{\Submanifold}$
  of
  $\apply{\ContinuousMap}{\Submanifold}$ such that
  $\SimplicialVolume{\TubularNeighborhood{\Submanifold}}$ vanishes and
  $
  \Manifold\setminus\TubularNeighborhood{\Submanifold}
  \cong
  \Manifold\setminus \Submanifold
  $%
\end{proposition}
\begin{proof}
  Let us denote $\apply{\ContinuousMap}{\Singularity_{mp}}$ by $\Singularity$.
  Then $\Singularity$ is a codimension $4$ submanifold. Additionally by the
  tranversality condition, the tangent spaces of the two preimages of a point
  in $\Singularity$ intersect a sphere of the fiber of the normal bundle of
  $\Singularity$ in a Hopf link.

  Let us denote a complement of a small tubular neighborhood of
  $\Singularity_{mp}$ by $\Submanifold^0$. Then
  $\apply{\ContinuousMap}{\Singularity_{mp}}$ is a codimension $2$-submanifold
  with boundary of $\Manifold$. The disk bundle of its normal bundle is a
  $\Ball{2}$-bundle over $\apply{\ContinuousMap}{\Singularity_{mp}}$. By
  \autoref{lem:FiberTransfer} it has vanishing simplicial volume.

  At the sphere of the normal bundle of a point of $\Singularity$ we are now
  given fundamental cycles of a tubular neighborhood of the two circles
  constituting the Hopf link and in order to obtain a fundamental cycle of the
  whole tubular neighborhood of $\apply{\ContinuousMap}{\Submanifold}$ we have
  to extend this to a fundamental cycle of the normal bundle of $\Singularity$.
  The construction of such an extension of arbitrarily small norm is
  completely analogous to the proof of
  \autoref{lem:FiberTransfer} using that the fundamental group of the
  complement of the Hopf link is abelian i.e. one first extends the given
  fundamental cycles to fundamental cycles of the sphere bundle of the
  normal bundle of $\Singularity$ and then extends these to the whole disk
  bundle of the normal bundle of $\Singularity$.
\end{proof}

==> Proposition/NeighborhoodImmersedSurface.tex <==
\begin{proposition}
\label{prp:TubNeighborhood}
  Let $\Manifold$ denote a $4$-manifold and $\Submanifold$ a possibly
  disconnected manifold of dimension $2$.
  Suppose we are given an immersion
  $
    \ContinuousMap
    \colon
    \Submanifold
    \to
    \Manifold
  $
  and a subset $\Singularity \subset \Submanifold$ that is the disjoint union
  of $\Singularity_{circ}$ and $\Singularity_{mp}$, such that
  \begin{itemize}
  \item
    The restriction of $\ContinuousMap$ to the complement of $\Singularity$ is
    an embedding,
  \item
    the images of $\Submanifold \setminus \Singularity$, $\Singularity_{circ}$
    and $\Singularity_{mp}$ are pairwise disjoint,
  \item
    $\Singularity_{circ}$ consists of embedded circles on which
    $\ContinuousMap$ is injective and the images of pairs of these circles
    either agree or are disjoint. If they agree, then the normal spaces at
    common points of these circles in $\Singularity_{circ}$ map to linearly
    independent lines in the normal bundle of the image in $\Manifold$,
  \item
    $\Singularity_{mp}$ is a discrete set and if the images of two points agree,
    then the tangent spaces
    of the two points intersect transversly
    in $\Tangenbundle{\Manifold}$.
  \end{itemize}
  then there exists a closed neighborhood $\TubularNeighborhood{\Submanifold}$
  of
  $\apply{\ContinuousMap}{\Submanifold}$ such that
  $\SimplicialVolume{\TubularNeighborhood{\Submanifold}}$ vanishes and
  $
    \Manifold\setminus\TubularNeighborhood{\Submanifold}
    \cong
    \Manifold\setminus \Submanifold
  $%
  .
\end{proposition}
\begin{proof}
  First of all note that if x$V_1$ and $V_2$ are codimension $2$ subspaces of
  $\Reals^n$ which intersect orthogonally, then the intersection of
  $
    V_1 \cup V_2
  $
  with $\Sphere{n-1}\subset \Reals^n$ is given by the product of the Hopf link
  and $\Sphere{n-4}$. By the
  aforementioned transversality condition we can pick neighborhoods $U_x\cong
  \Reals^4$ for all $x\in \apply{\ContinuousMap}{\Singularity}$ such that in
  $U_x$ the immersion $\ContinuousMap$ looks like the inclusion of two
  orthogonal $2$-planes.

  Let us now fix a metric on $\Manifold$ and then let
  $\pi\colon\NormalBundle{\Submanifold}{\ContinuousMap}\to \Submanifold$ denote
  the $\Ball{2}$-normal
  bundle of $\ContinuousMap$ i.e. the pullback of the pointwise underlying disk
  bundle of the orthogonal complement of the image of the differential.
  We can extend $\ContinuousMap$ to
  $\NormalBundle{\Submanifold}{\ContinuousMap}$ so that this extension is
  locally a tubular neighborhood.
  Let us fix a small neighborhood $V$ of $\Singularity\subset \Submanifold$
  consisting of balls and
  let us additionally assume that
  $
    \apply
      {\ContinuousMap}
      {\at{\NormalBundle{\Submanifold}{\ContinuousMap}}{V}}
    =
    \bigsqcup U_x
  $.

  We will first construct a fundamental cycle of arbitrarily small norm
  $\FundamentalCycle{\Submanifold\setminus V}$ for
  $
    \at
      {\NormalBundle{\Submanifold}{\ContinuousMap}}
      {\Submanifold\setminus V}
  $
  such that $\Boundary{\FundamentalCycle{\Submanifold\setminus V}}$ is a sum of
  a fundamental cycle for the underlying $\Sphere{1}$-bundle of
  $
    \at
      {\NormalBundle{\Submanifold}{\ContinuousMap}}
      {\Submanifold\setminus V}
  $
  and a fundamental cycle for
  $
    \at
      {\NormalBundle{\Submanifold}{\ContinuousMap}}
      {\Boundary{V}}
  $
  and then we will extend this cycle to $\bigsqcup U_x$ in a controlled fashion.

  Fix a fundamental cycle
  $\FundamentalCycle{\Submanifold\setminus\Inner{V},\Boundary{V}}$ and let us
  use Lemma~\ref{lem:FiberTransfer} to define
  \[
    \FundamentalCycle
      {\at
          {\NormalBundle{\Submanifold}{\ContinuousMap}}
          {\Submanifold\setminus V}
      }
    \coloneqq
    \apply
      {\FiberTransferHomology{\pi}}
      {\FundamentalCycle{\Submanifold\setminus\Inner{V,\Boundary{V}}}}
  \]
  Note that
  $
    \FundamentalCycle
      {
        \at
          {\NormalBundle{\Submanifold}{\ContinuousMap}}
          {\Submanifold\setminus V}
      }
  $
  can be chosen to have arbitrarily small norm.
  Now
  $
    \apply
      {\FiberTransferHomology{\pi}}
      {
        \Boundary
          {\FundamentalCycle{\Submanifold\setminus\Inner{V},\Boundary{V}}}
      }
  $
  yields a representative of arbitrarily small norm of the fundamental class of
  the neighborhood of the Hopf links in $\Boundary{U_x}\cong \Sphere{3}$. Hence
  $
    \Boundary
      {\apply
        {\FiberTransferHomology{\pi}}
        {
          \Boundary
          {\FundamentalCycle{\Submanifold\setminus\Inner{V},\Boundary{V}}}
        }
      }
  $
  yields a representative of arbitrarily small norm of the fundamental cycles
  of the boundary of $\Sphere{3}\setminus \Inner{N}$, where $N$ denotes a
  neighborhood of the Hopf link. Since the complement of the Hopf Link has
  fundamental group $\Integers^2$, the cycle
  $
    \Boundary
      {\apply
        {\FiberTransferHomology{\pi}}
        {
          \Boundary
          {\FundamentalCycle{\Submanifold\setminus\Inner{V},\Boundary{V}}}
        }
      }
  $
  bounds a fundamental cycle of $(\Sphere{3} \setminus \Inner{N},\Boundary{N})$
  of arbitrarily small norm. All in all this shows that
  $
    \apply
      {\FiberTransferHomology{\pi}}
      {
        \Boundary
        {\FundamentalCycle{\Submanifold\setminus\Inner{V},\Boundary{V}}}
      }
  $
  can be extended to yield arbitrarily small representatives of the fundamental
  class of $\bigsqcup\Boundary{U_x}$. Adding the cones of these representatives
  in $\bigsqcup U_x \cong \bigsqcup \Ball{4}$ to
  $
    \FundamentalCycle
      {\at
        {\NormalBundle{\Submanifold}{\ContinuousMap}}
        {\Submanifold\setminus V}
      }
  $
  yields a representative of arbitrarily small norm of a tubular neighborhood
  of $\apply{\ContinuousMap}{\Submanifold}$
\end{proof}

==> Proposition/NonZeroBoundedCohomology.tex <==
\begin{proposition}
\label{prp:Splitting}
  Let $\Manifold$ denote a closed manifold of dimension $n$ with non-zero
  simplicial volume.
  Suppose further that there exists a codimension $0$ submanifold with boundary
  $\Manifold'\subset \Manifold$ such that the simplicial volume of
  $(\Manifold',\Boundary{\Manifold'})$ vanishes. Then the $n$-th bounded
  cohomology of
  $\HomotopyGroupOfObject{1}{\Manifold\setminus\Manifold'}{\ast}$ is non-zero.
\end{proposition}

==> Proposition/OpenBookVanishingWithoutAssumption.tex <==
\begin{proposition}
\label{prp:OpenBookVanishingWithout}
  Let $\Manifold$ denote a $4$-manifold which admits an open book decomposition
  such that its hyperbolic pieces admit only toroidal boundaries, then the
  simplicial volume of $\Manifold$ vanishes.

  In particular if the binding only
  contains spheres and tori, then the simplicial volume of $\Manifold$ vanishes.
\end{proposition}

==> Proposition/SurfaceGroupsAndFiberingGroups.tex <==
\begin{proposition}
  The $n$-th bounded cohomology of a non-abelian surface group
  $\SurfaceGroup{g}$ is non-zero if and only if the $n$-th bounded cohomology
  of non-abelian free groups is non-zero.

  If the $n$-th bounded cohomology of a surface group is zero, then the
  $n$-th bounded cohomology of all fibering $3$-manifold groups vanishes.
\end{proposition}
\begin{proof}
  It was proven in \cite{Bouarich} that if one has a short exact sequence of
  groups
  \[
    1 \to \Subgroup \to \Group \to \AmenableGroup\to 1
  \]
  where $\AmenableGroup$ is amenable, then the bounded cohomology of
  $\Group$ agrees with the $\AmenableGroup$-invarians of the bounded cohomology
  of $\Subgroup$. In particular the inclusion $\Subgroup \to \Group$ induces an
  injection in bounded cohomology.

  Since the fundamental group $\Group$ of a fibering $3$-manifold fits into an
  exact sequence
  \[
    1 \to \SurfaceGroup{g} \to \Group \to \Integers
  \]
  the second claim follows. Additionally note that the commutator subgroup of a
  non-abelian surface group is an infinitely generated free group, which yields
  half of the first claim. For the other half notice that there is a surjection
  $
    \SurfaceGroup{g}
    \to
    \FreeGroup{g}
  $
  which splits and hence the bounded cohomology of $\FreeGroup{g}$ embeds into
  the bounded cohomology of $\SurfaceGroup{g}$.
\end{proof}

==> Section/Codim.tex <==
\label{scn:Codim}
The goal of the following section is to establish vanishing results for tubular
neighborhoods of various codimension $2$ submanifolds.
In light of \autoref{prp:Splitting} such results yield
\autoref{thm:ImmersedKnotsEtc}.

Since tubular neighborhoods airse from normal bundles, we will construct
fundamental cycles by realizing the fiber transfer on the chain level.

The fiber transfer is sometimes called the Gysin map or the Umkehr map. There
are various definitions some more geometric, some more algebraic in flavor. We
will use the following:
Let $\FiberingProjektion{\ManifoldTotal}\colon\ManifoldTotal \to \ManifoldBase$
denote a fiber bundle of oriented
manifolds with fiber $\ManifoldFiber$ of dimension $\FiberDimension$. Then
$
  \FiberTransferHomology{\FiberingProjektion{\ManifoldTotal}}
  \colon
  \HomologyOfSpaceObject{*}{\ManifoldBase}{\Integers}
  \to
  \HomologyOfSpaceObject{*+\FiberDimension}{\ManifoldTotal}{\Integers}
$
is defined by
\[
  \apply
    {\FiberTransferHomology{\FiberingProjektion{\ManifoldTotal}}}
    {\HomologyClass}
  =
  \apply
    {PD \circ \FiberingProjektion{\ManifoldTotal}^* \circ PD^{-1}}
    {\HomologyClass}
\]
where $PD$ denotes the Poincare duality isomorphism.
Assume that $\HomologyClass$ is
$\apply{\HomologyOfSpaceMorphism{\ContinuousMap}}{\FundamentalClass{\Manifold}}$
for $\ContinuousMap \colon \Manifold \to \ManifoldBase$ some map of closed
manifolds, then one easily checks that
$
  \apply
    {\FiberTransferHomology{\FiberingProjektion{\ManifoldTotal}}}
    {\HomologyClass}
  =
  \apply
    {\HomologyOfSpaceMorphism{\overline{\ContinuousMap}}}
    {\FundamentalClass{\ContinuousMap^! \ManifoldTotal}}
$
where $\overline{\ContinuousMap}$ denotes the induced map from the pullback
$\ContinuousMap^! \ManifoldTotal$ to $\ManifoldTotal$.

The following lemma can be understood as an extension of (CITE GROMOV FIBER
RESULT \cite{GRomov?})
\input{Lemma/FiberTransfer.tex}
In the general case we have the following proposition that can be further
strengthened in dimension $4$.
\input{Proposition/NeighborhoodImmersedCodim2.tex}
In dimension $4$ there are less requirements on the self intersections of
the submanifold. In particular the map does not necessarily have to be
self-transverse everywhere.
\input{Proposition/NeighborhoodImmersedSurface.tex}
Together with \autoref{prp:Splitting} this yields:
\input{Theorem/GeneralizedKnots.tex}

==> Section/Preliminaries.tex <==
\label{scn:BCofFreeGroups}
The following section recalls some facts about bounded cohomology of free
groups.
Let $\FreeGroup{n}$ denote the free group on $n$-generators.
\input{Proposition/FreeGroupRankIrrelevant.tex}
\input{Proposition/SurfaceGroupsAndFiberingGroups.tex}


==> Section/Signature.tex <==
\label{scn:Signature}
The reader is advised to consult Section~29 in \cite{Ranicki} or \cite{Quinn}
for a thorough introduction to the asymmetric signature as this short section
is only intended for the computation that the asymetric signature of the
product of two surfaces vanishes.

Let $\Group$ denote a group and $\IntegralGroupRing{\Group}$ the corresponding
integral group ring. We call a $V$ denote a finitely generated, projective
$\IntegralGroupRing{\Group}$-module together with an isomorphism $\lambda\colon
V \to V^*$ a \introduce{form over $\IntegralGroupRing{\Group}$}.

We call a submodule $L \subset V$ a \introduce{Lagrangian}, if the sequence
\[
  0
  \to
  L
  \to
  V
  \to
  L^*
  \to
  0
\]
is exact. Here the map $V \to L^*$ is defined by the composition of the
$\lambda$ and the dual of the inclusion of $L$ to $V$.

We define the \introduce{Witt group of $\IntegralGroupRing{\Group}$}, denoted by
$\apply{W_p}{\IntegralGroupRing{\Group}}$,
as the free abelian group generated by forms over $\IntegralGroupRing{\Group}$
modulo the forms containing a Lagrangian.

Now given a closed, $n$-dimensional, triangulated manifold $\Manifold$ with
fundamental group
$\Group$, one can endow the integral simplicial chain complex
$\apply{C_*}{\UniversalCovering{\Manifold}}$ with the structure of a free and
based $\IntegralGroupRing{\Group}$-module. We denote by
$\apply{C^*}{\UniversalCovering{\Manifold}}$ the cochain complex
$
  \apply
    {\mathrm{Hom}_{\IntegralGroupRing{\Group}}}
    {
      \apply{C_*}{\UniversalCovering{\Manifold}}
      ,
      \IntegralGroupRing{\Group}
    }
$%
. It is shown in Section~2 of \cite{Wall} that the cap product with a
fundamental cycle $\FundamentalCycle{\Manifold}$ of $\Manifold$ induces a chain
homotopy equivalence
\[
  \FundamentalCycle{\Manifold} \cap -
  \colon
  \apply{C^*}{\UniversalCovering{\Manifold}}
  \to
  \apply{C_{n-*}}{\UniversalCovering{\Manifold}
\]

==> Section/reducible.tex <==
In this appendix we will present the proof of \cite{Mccullough} of a theorem
that was originally proven by De Sà in \cite{DeSaThesis}. Since both only state
the theorem for $3$-manifolds without boundary (although De Sà states in
Remark~c) before Corollary~3.2 in \cite{DeSaThesis} that the theorem can
analogously be adapted to the bounded case) and we use the case of
$3$-manifolds with boundary, we include McCulloughs proof to show that it also
applies in the bounded case.

Let $\Manifold$ denote a $3$-manifold with possible non-empty boundary and let
$\Diffeomorphism$ denote a diffeomorphism of $\Manifold$ that restricts to the
identity on its boundary. Then according to Theorem~3.1 in \cite{Bonahon} there
exists a set $\Sigma \subset \Manifold$ consisting of embedded, separating
$2$-spheres, such that if $\Manifold_0, \ldots , \Manifold_n$ denotes the
connected components of $\Manifold \setminus \Sigma$, then $\Manifold_0$ is a
the complement of $n$ points in $\Sphere{3}$ and each $\Manifold_{i}$ meets a
unique component of $\Sigma$ and furthermore any embedded $2$-sphere in the
manifolds $\Manifold_{i}$ for $i \geq 1$ either bounds a $3$-ball or is
boundary parallel.

\input{Theorem/ReducibleDiffeo.tex}

==> Section/strategy.tex <==
In this section we establish a connection between simplicial volume, bounded
cohomology and splitting a manifold into two parts. The general idea can be
paraphrased as follows: If an $n$-dimensional manifold with non-zero simplicial
volume can be split in two parts, one of which has vanishing simplicial volume,
then the other part has to have non-zero $n$-th bounded cohomology.

The connection is based on the following definition by Matsumoto and Morita.
\input{Definition/UBC.tex}
The uniform boundary condition is closely tied to bounded cohomology via the
following proposition:
\input{Proposition/MatsumotoMorita.tex}
Note that by Gromovs Mapping Theorem the bounded cohomology of a connected
topological space agrees with the bounded cohomology of its fundamental group.
Hence we obtain the following corollary:
\input{Corollary/AcyclicImpliesUBC.tex}
We will be interested in constructing fundamental cycles. For that we need the
following lemma:
\input{Lemma/BoundingCycle.tex}
Using this lemma together with the uniform boundary condition yields the
following elementary observation about simplicial volume:
\input{Lemma/UBCimpliesSimplicialVolume.tex}
Combining this lemma with Proposition~\ref{prp:MatsumotoMorita} yields as an
immediate consequence the following proposition:
\input{Proposition/NonZeroBoundedCohomology.tex}

==> Theorem/BoundedCohomologyFreeGroupNonZero.tex <==
\begin{theorem}
  For all $n\geq 4$, there exists a $k\geq 2$, such that
  $\BoundedCohomologyOfSpaceObject{n}{\FreeGroup{k'}}{\Reals}$ is non-zero for
  all $k'\geq k$.
\end{theorem}
\begin{proof}
  Proposition~\ref{prp:Existence} and Lemma~\ref{lem:FreeGroupUBC} imply that
  that for all $n\geq 4$, there exists some $k\geq 2$ such that
  $
    \BoundedCohomologyOfSpaceObject{n}{\FreeGroup{k}}{\Reals}
  $
  is non-zero.
  Since $\FreeGroup{k}$ is a retract of $\FreeGroup{k'}$ for $k'\geq k$, this
  implies that
  $
    \BoundedCohomologyOfSpaceObject{n}{\FreeGroup{k'}}{\Reals}
  $ is also non-zero for all $k'\geq k$.
\end{proof}

==> Theorem/FourthBC.tex <==
\begin{theorem}
  Bounded cohomology in degree four of non-abelian free groups does not vanish.
\end{theorem}

==> Theorem/GeneralizedKnots.tex <==
\begin{theorem}
\label{thm:ImmersedKnotsEtc}
  Let $\Manifold$ denote an $n$-dimensional manifold with non-zero simplicial
  volume and let
  $
    \ContinuousMap
    \colon
    \Submanifold^{n-2}
    \to
    \Manifold^n
  $
  denote a map satisfying the hypothesis of
  \autoref{prp:GeneralizedTubNeighborhood} or if $n=4$ the
  hypothesis fo \autoref{prp:TubNeighborhood}, then
  the $n$-th bounded cohomology of $\Manifold \setminus
  \apply{\ContinuousMap}{\Submanifold}$ is non-zero.
\end{theorem}

==> Theorem/KnotsIntroduction.tex <==
\begin{theorem}
  Let $\Manifold$ denote an $n$-dimensional manifold of non-zero simplicial
  volume. and let $\Submanifold \subset \Manifold$ denote a submanifold of
  codimension two, then the $n$-th bounded cohomology of $\Manifold \setminus
  \Submanifold$ is non-zero.
  If $n=4$, then $\Submanifold$ is allowed to have self-transversal
  self-intersections.
\end{theorem}

==> Theorem/ReducibleDiffeo.tex <==
\begin{theorem}[Theorem~Something in \cite{McCullough}]
\label{thm:ReducibleDiffeo}
\end{theorem}
